Hexatagging: Projective Dependency Parsing as Tagging

We introduce a novel dependency parser, the hexatagger, that constructs dependency trees by tagging the words in a sentence with elements from a finite set of possible tags. In contrast to many approaches to dependency parsing, our approach is fully parallelizable at training time, i.e., the structure-building actions needed to build a dependency parse can be predicted in parallel to each other. Additionally, exact decoding is linear in time and space complexity. Furthermore, we derive a probabilistic dependency parser that predicts hexatags using no more than a linear model with features from a pretrained language model, i.e., we forsake a bespoke architecture explicitly designed for the task. Despite the generality and simplicity of our approach, we achieve state-of-the-art performance of 96.4 LAS and 97.4 UAS on the Penn Treebank test set. Additionally, our parser's linear time complexity and parallelism significantly improve computational efficiency, with a roughly 10-times speed-up over previous state-of-the-art models during decoding.

==> algs/def_tree.tex <==
\newcommand{\NTx}[0]{\textrm{X}[x]}

\newcommand{\newlextree}[0]{%
\small
\begin{tikzpicture}[baseline=1ex,x=0.05\linewidth, y=0.04\linewidth][%
\draw[] (3.0, 2.) node[shape=ellipse,inner sep=0pt,black] (N1) {\tiny $\NTx$};

\draw[] (0., 0.) node[shape=rectangle,black,thick,inner sep=0pt] (C1) {\tiny $\calT_1$};
\draw[] (1., 0.) node[shape=rectangle,black,thick,inner sep=0pt] (C2) {\tiny $\calT_2$};
\draw[] (2.2, 0.) node[shape=rectangle,black,thick,inner sep=0pt] (C3) {\tiny $\cdots$};

\draw[] (3.4, 0.) node[shape=rectangle,blue,draw,thick,inner sep=2.5pt] (C4) {\tiny $x$};
% \draw[] (3.4, 0.) node[shape=rectangle,black,thick,inner sep=1pt] (C4) {\tiny $x$};

\draw[] (4.8, 0.) node[shape=rectangle,black,thick,inner sep=0pt] (C3) {\tiny $\cdots$};
\draw[] (6.8, -0.1) node[shape=rectangle,black,thick,inner sep=1pt] (C5) {\tiny $\calT_{\displaystyle |N_{\displaystyle \calG}(x)|}$};

\draw[thick,black] (N1) -- (C1);
\draw[thick,black] (N1) -- (C2);
\draw[thick,black] (N1) -- (C4);
\draw[thick,black] (N1) -- (C5);
\end{tikzpicture}}



\newcommand{\newbintreeL}[0]{%
\small
\begin{tikzpicture}[baseline=-2ex,x=0.04\linewidth, y=0.05\linewidth][%
\draw[] (3.0, 2.) node[shape=circle,draw,thick,inner sep=1pt] (N1) {\tiny L};

\draw[] (1.5, 0.5) node[shape=circle,draw,thick,inner sep=1pt] (L2) {\tiny L};
\draw[] (4.8, 0.3) node[shape=rectangle,black,thick,inner sep=0pt] (R2) {\tiny $\calT_{\displaystyle |N_{\calG}(x)|}$};

\draw[] (0.,-1.) node[shape=rectangle,black,thick,inner sep=1pt] (L3) {\tiny $\cdots$};
\draw[] (3.8,-1.3) node[shape=rectangle,black,thick,inner sep=0pt] (R3) {\tiny $\calT_{\displaystyle |N_{\calG}(x)|\mathbin{-1}}$};

\draw[] (-1.3,-2.8) node[shape=rectangle,black,thick,inner sep=0pt] (L4) {\tiny $\calT_1$};
\draw[] (1.3,-2.8) node[shape=circle,draw,thick,inner sep=1pt] (R4) {\tiny R};

\draw[] (0.2,-4.3) node[shape=rectangle,black,thick,inner sep=0pt] (L5) {\tiny $\calT_2$};
\draw[] (2.8,-4.3) node[shape=rectangle,black,thick,inner sep=1pt] (R5) {\tiny $\cdots$};

\draw[] (1.7,-5.8) node[shape=rectangle,black,thick,inner sep=0pt] (L6) {\tiny $\calT_{n-1}$};
\draw[] (4.3,-5.8) node[shape=rectangle,blue,draw,thick,inner sep=2.5pt] (R6) {\tiny $x$};


\draw[thick,black] (N1) -- (L2);
\draw[thick,black] (N1) -- (R2);

\draw[thick,black] (L2) -- (L3);
\draw[thick,black] (L2) -- (R3);

\draw[thick,black] (L3) -- (L4);
\draw[thick,black] (L3) -- (R4);

\draw[thick,black] (R4) -- (L5);
\draw[thick,black] (R4) -- (R5);

\draw[thick,black] (R5) -- (L6);
\draw[thick,black] (R5) -- (R6);
\end{tikzpicture}}


\newcommand{\newbintreeR}[0]{%
\small
\begin{tikzpicture}[baseline=-2ex,x=0.04\linewidth, y=0.0475\linewidth][%
\draw[] (3.5, 2.) node[shape=circle,draw,thick,inner sep=1pt] (N1) {\tiny R};

\draw[] (2.2, 0.3) node[shape=rectangle,black,thick,inner sep=0pt] (L2) {\tiny $\calT_1$};
\draw[] (5.0, 0.5) node[shape=circle,draw,thick,inner sep=1pt] (R2) {\tiny R};

\draw[] (3.6,-1.) node[shape=rectangle,black,thick,inner sep=0pt] (L3) {\tiny $\calT_2$};
\draw[] (6.2,-1.) node[shape=rectangle,black,thick,inner sep=1pt] (R3) {\tiny $\cdots$};

\draw[] (4.8,-2.8) node[shape=circle,draw,thick,inner sep=1pt] (L4) {\tiny L};
\draw[] (8.0,-3.0) node[shape=rectangle,black,thick,inner sep=0pt] (R4) {\tiny $\calT_{\displaystyle |N_{\calG}(x)|}$};

\draw[] (3.3,-4.3) node[shape=rectangle,black,thick,inner sep=1pt] (L5) {\tiny $\cdots$};
\draw[] (6.6,-4.5) node[shape=rectangle,black,thick,inner sep=0pt] (R5) {\tiny $\calT_{\displaystyle |N_{\calG}(x)|\mathbin{-1}}$};

\draw[] (2.0,-5.8) node[shape=rectangle,blue,draw,thick,inner sep=2.5pt] (L6) {\tiny $x$};
\draw[] (4.8,-6.0) node[shape=rectangle,black,thick,inner sep=2pt] (R6) {\tiny $\calT_{n+1}$};



\draw[thick,black] (N1) -- (L2);
\draw[thick,black] (N1) -- (R2);

\draw[thick,black] (R2) -- (L3);
\draw[thick,black] (R2) -- (R3);

\draw[thick,black] (R3) -- (L4);
\draw[thick,black] (R3) -- (R4);

\draw[thick,black] (L4) -- (L5);
\draw[thick,black] (L4) -- (R5);

\draw[thick,black] (L5) -- (L6);
\draw[thick,black] (L5) -- (R6);
\end{tikzpicture}}


==> algs/dep2pbt.tex <==
% algorithm for converting dependency graph to lexicalized tree

\begin{algorithm}[!h]
\caption{Transforming a dependency graph $\calG$ to a pivot binary tree $\calT$.} 
\hspace*{\algorithmicindent} \textbf{Input} Dependency graph $\calG_{\texttt{root}}$ with root node \texttt{root} (i.e., the unique node with no incident edges) \\
\hspace*{\algorithmicindent} \textbf{Output} Pivot binary tree $\calT$
% \hspace*{\algorithmicindent} \textbf{Prerequisite} 
\begin{algorithmic}[1]
    \footnotesize
    \Procedure{Dep2pbt}{$\calG_{\texttt{root}}$}
    \State $x \gets \texttt{root}$ \Comment{Initializing $x$ to the \texttt{root} node in the dependency graph $\calG$}
    \For{$x_i \in N_{\calG}(x)$} \Comment{$N_{\calG}(x)$ is the set of neighboring nodes (dependents) of x, ordered by their positions in the input sentence}
        \State $\calT_i \gets$ \textsc{Dep2pbt}$ \big( \calG_{x_i} \big) $
    \EndFor 
    \State $\calT \gets \textsc{Lex2bin} \left( \newlextree \right)$
    \vspace{3pt}
    \State \Return $\calT$
    
    \EndProcedure
\end{algorithmic}\label{alg:dep2pbt}
\end{algorithm}

==> algs/lex2bin.tex <==
% algorithm for binarizing a lexicalized tree to
\begin{algorithm}[!h]
\caption{Binarization of a lexicalized subtree $\calT$.} \label{alg:lex2bin-tree}
\hspace*{\algorithmicindent} \textbf{Input} Lexicalized subtree $\calT$ with $N_{\calG}(x)$ child nodes, in which the $n$-th is the head $x$ \\
\hspace*{\algorithmicindent} \textbf{Output} Pivot binary subtree $\calT^{B}$
\begin{algorithmic}[1]
    \footnotesize
    \Procedure{Lex2bin}{$\calT$}
    \vspace{3pt}
        \State  $\calT^{B} \gets \underbrace{\newbintreeL}_{\textsc{Left-first}}$ \;or\; $\underbrace{\newbintreeR}_{\textsc{Right-first}}$ 
    \vspace{2pt}
    \State \Return $\calT^{B}$
    \EndProcedure
\end{algorithmic}
\end{algorithm}


==> figs/def_derivation.tex <==
%%% This code is taken from Nikita's tetra-tagging paper
%%%

%%% Figures used to represent the stack at various points in the example derivation

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Single terminal nodes with a parent
\newcommand{\newstacka}[0]{%
\small
\begin{tikzpicture}[x=0.05\linewidth, y=0.05\linewidth][%
\draw[] (1.5, 1.5) node[shape=circle,thick,inner sep=0pt,blue] (N1) {\tt \$};

\draw[] (0.3, 0.5) node[shape=rectangle,blue,draw,thick,inner sep=2pt] (NA) {A};

\draw[thick,blue] (NA) -- (N1);
\end{tikzpicture}}

\newcommand{\newdepa}[0]{%
\begin{dependency}[baseline=-1ex,x=0.05\linewidth, y=0.05\linewidth,arc edge, arc angle=50, text only label, label style={above}]
\begin{deptext}[column sep=.13cm]
A  \\
\end{deptext}
\end{dependency}}

\newcommand{\newstackb}[0]{%
\small
\begin{tikzpicture}[x=0.05\linewidth, y=0.05\linewidth][%
\draw[] (1.5, 1.5) node[shape=circle,thick,inner sep=0pt,blue] (N1) {\tt \$};

\draw[] (0.3, 0.5) node[shape=rectangle,blue,draw,thick,inner sep=2pt] (NA) {B};

\draw[thick,blue] (NA) -- (N1);
\end{tikzpicture}}

\newcommand{\newstackc}[0]{%
\small
\begin{tikzpicture}[x=0.05\linewidth, y=0.05\linewidth][%
\draw[] (1.5, 1.5) node[shape=circle,thick,inner sep=0pt,blue] (N1) {\tt \$};

\draw[] (0.3, 0.5) node[shape=rectangle,blue,draw,thick,inner sep=2pt] (NA) {C};

\draw[thick,blue] (NA) -- (N1);
\end{tikzpicture}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\newstackaa}[0]{%
\small
\begin{tikzpicture}[x=0.05\linewidth, y=0.05\linewidth][%
\draw[] (1.5, 1.5) node[shape=circle,blue,draw,thick,inner sep=1pt] (N1) {R};
\draw[] (2.7, 0.3) node[blue,inner sep=1pt] (N2) {$\varnothing$};

\draw[] (2.5, 2.5) node[blue,inner sep=0pt] (N4) {\tt \$};

\draw[] (0.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NA) {A};

\draw[thick] (NA) -- (N1);
\draw[thick,blue] (N1) -- (N4);
\draw[thick,blue] (N2) -- (N1);
\end{tikzpicture}}

\newcommand{\newdepaa}[0]{%
\begin{dependency}[baseline=-1ex,x=0.05\linewidth, y=0.05\linewidth,arc edge, arc angle=50, text only label, label style={above}, edge horizontal padding=3pt]
\begin{deptext}[column sep=.13cm]
A  \\
\end{deptext}
\deproot[edge height=4ex,blue]{1}{}
\end{dependency}}

%%%%%

\newcommand{\stackaa}[0]{%
\small
\begin{tikzpicture}[x=0.05\linewidth, y=0.05\linewidth][%
\draw[] (1.5, 1.5) node[shape=circle,draw,thick,inner sep=1pt] (N1) {R};
\draw[] (2.7, 0.3) node[inner sep=1pt] (N2) {$\varnothing$};

\draw[] (2.5, 2.5) node[inner sep=0pt] (N4) {\tt \$};

\draw[] (0.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NA) {A};

\draw[thick] (NA) -- (N1);
\draw[thick] (N1) -- (N4);
\draw[thick] (N2) -- (N1);
\end{tikzpicture}}

%%%%%

\newcommand{\newstackaab}[0]{%
\small
\begin{tikzpicture}[x=0.05\linewidth, y=0.05\linewidth][%
\draw[] (1.5, 1.5) node[shape=circle,draw,thick,inner sep=1pt] (N1) {L};
\draw[] (2.5, 2.5) node[inner sep=0pt] (N4) {\tt \$};
\draw[] (0.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NA) {A};

\draw[] (2.7, 0.3) node[shape=rectangle,blue,draw,thick,inner sep=2pt] (N2) {B};
\draw[] (3.7, 1.3) node[blue,inner sep=0pt] (N5) {\tt \$};


\draw[thick] (NA) -- (N1);
\draw[thick,blue] (N1) -- (N4);

\draw[thick,blue] (N2) -- (N5);
\end{tikzpicture}}


\newcommand{\newdepaab}[0]{%
\begin{dependency}[baseline=-1ex,x=0.05\linewidth, y=0.05\linewidth,arc edge, arc angle=50, text only label, label style={above}, edge horizontal padding=3pt]
\begin{deptext}[column sep=.13cm]
A  \& {\color{blue} B} \\
\end{deptext}
\deproot[edge height=4ex]{1}{}
\end{dependency}}

%%%%%

\newcommand{\newstackaabb}[0]{%
\small
\begin{tikzpicture}[x=0.05\linewidth, y=0.05\linewidth][%
\draw[] (1.5, 2.5) node[shape=circle,draw,thick,inner sep=1pt] (N1) {R};
\draw[] (3.5, 1.5) node[shape=circle,blue,draw,thick,inner sep=1pt] (N2) {L};
\draw[] (4.7, 0.3) node[blue,inner sep=1pt] (N3) {$\varnothing$};
\draw[] (2.5, 3.5) node[inner sep=0pt] (N4) {\tt \$};

\draw[] (0.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NA) {A};
\draw[] (2.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NB) {B};

\draw[thick] (NA) -- (N1);
\draw[thick] (NB) -- (N2);
\draw[thick] (N1) -- (N4);
\draw[thick,blue] (N2) -- (N1);
\draw[thick,blue] (N3) -- (N2);
\end{tikzpicture}}


\newcommand{\stackaabb}[0]{%
\small
\begin{tikzpicture}[x=0.05\linewidth, y=0.05\linewidth][%
\draw[] (1.5, 2.5) node[shape=circle,draw,thick,inner sep=1pt] (N1) {R};
\draw[] (3.5, 1.5) node[shape=circle,draw,thick,inner sep=1pt] (N2) {L};
\draw[] (4.7, 0.3) node[inner sep=1pt] (N3) {$\varnothing$};
\draw[] (2.5, 3.5) node[inner sep=0pt] (N4) {\tt \$};

\draw[] (0.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NA) {A};
\draw[] (2.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NB) {B};

\draw[thick] (NA) -- (N1);
\draw[thick] (NB) -- (N2);
\draw[thick] (N1) -- (N4);
\draw[thick] (N2) -- (N1);
\draw[thick] (N3) -- (N2);
\end{tikzpicture}}

\newcommand{\newdepaabb}[0]{%
\begin{dependency}[baseline=-1ex,x=0.05\linewidth, y=0.05\linewidth,arc edge, arc angle=50, text only label, label style={above}, edge horizontal padding=3pt]
\begin{deptext}[column sep=.13cm]
A  \&  B  \\
\end{deptext}
\deproot[<-,blue,edge height=4ex]{2}{}
% \deproot[->,blue,edge below,edge height=-1ex]{2}{}
\depedge[blue,edge height=4ex]{2}{1}{}
\end{dependency}}

%%%%%

\newcommand{\newdepaabbc}[0]{%
\begin{dependency}[baseline=-1ex,x=0.05\linewidth, y=0.05\linewidth,arc edge, arc angle=50, text only label, label style={above}, edge horizontal padding=3pt]
\begin{deptext}[column sep=.13cm]
A  \& B \& {\color{blue} C} \\
\end{deptext}
\deproot[<-,edge height=4ex]{2}{}
\depedge{2}{1}{}
\end{dependency}}

%%%


\newcommand{\newstackaabbcc}[0]{%
\small
\begin{tikzpicture}[x=0.05\linewidth, y=0.05\linewidth][%
\draw[] (1.5, 3.5) node[shape=circle,draw,thick,inner sep=1pt] (N1) {R};
\draw[] (3.5, 2.5) node[shape=circle,draw,thick,inner sep=1pt] (N2) {L};
\draw[] (5.5, 1.5) node[shape=circle,draw,blue,thick,inner sep=1pt] (N3) {R};
\draw[] (2.5, 4.5) node[inner sep=0pt] (N4) {\tt \$};

\draw[] (0.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NA) {A};
\draw[] (2.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NB) {B};
\draw[] (4.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NC) {C};
\draw[] (6.5, 0.3) node[blue,inner sep=1pt] (ND) {$\varnothing$};

\draw[thick] (NA) -- (N1);
\draw[thick] (NB) -- (N2);
\draw[thick] (NC) -- (N3);
\draw[thick,blue] (ND) -- (N3);
\draw[thick] (N1) -- (N4);
\draw[thick] (N2) -- (N1);
\draw[thick,blue] (N3) -- (N2);
\end{tikzpicture}}

\newcommand{\newdepaabbcc}[0]{%
\begin{dependency}[baseline=-1ex,x=0.05\linewidth, y=0.05\linewidth,arc edge, arc angle=50, text only label, label style={above}, edge horizontal padding=3pt]
\begin{deptext}[column sep=.13cm]
A  \& B \&  C \\
\end{deptext}
\deproot[<-,edge height=4ex]{2}{}
\deproot[->,blue,edge height=4ex]{3}{}
\depedge[]{2}{1}{}

\end{dependency}}

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%


\newcommand{\newstackaabbccd}[0]{%
\small
\begin{tikzpicture}[x=0.05\linewidth, y=0.05\linewidth][%
\draw[] (1.5, 3.5) node[shape=circle,draw,thick,inner sep=1pt] (N1) {R};
\draw[] (3.5, 2.5) node[shape=circle,draw,thick,inner sep=1pt] (N2) {L};
\draw[] (5.5, 1.5) node[shape=circle,draw,thick,inner sep=1pt] (N3) {R};
\draw[] (2.5, 4.5) node[inner sep=0pt] (N4) {\tt \$};

\draw[] (0.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NA) {A};
\draw[] (2.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NB) {B};
\draw[] (4.5, 0.3) node[shape=rectangle,draw,thick,inner sep=2pt] (NC) {C};
\draw[] (6.5, 0.3) node[shape=rectangle,draw,blue,thick,inner sep=2pt] (ND) {D};

\draw[thick] (NA) -- (N1);
\draw[thick] (NB) -- (N2);
\draw[thick] (NC) -- (N3);
\draw[thick,blue] (ND) -- (N3);
\draw[thick] (N1) -- (N4);
\draw[thick] (N2) -- (N1);
\draw[thick] (N3) -- (N2);
\end{tikzpicture}}


\newcommand{\newdepaabbccd}[0]{%
\begin{dependency}[baseline=-1ex,x=0.05\linewidth, y=0.05\linewidth,arc edge, arc angle=50, text only label, label style={above}, edge horizontal padding=3pt]
\begin{deptext}[column sep=.13cm]
A  \& B \& C \& {\color{blue} D} \\
\end{deptext}
\depedge{2}{1}{}
\depedge[blue]{2}{4}{}
\depedge[blue]{4}{3}{}
\deproot[->,red,edge height=5ex]{2}{root}
\end{dependency}}
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%

\newcommand{\dashrule}[1][black]{%
  \color{#1}\rule[\dimexpr.5ex-.2pt]{4pt}{.4pt}\xleaders\hbox{\rule{4pt}{0pt}\rule[\dimexpr.5ex-.2pt]{4pt}{.4pt}}\hfill\kern0pt%
}
\newcommand{\mydashrule}[0]{%
\\[-2\jot]
\multicolumn{4}{@{}c@{}}{\makebox[\linewidth]{\dashrule[black!60]}} \\[-\jot]}


\newcommand{\thickdashrule}[1][black]{%
  \color{#1}\rule[\dimexpr.5ex-.2pt]{4pt}{1.2pt}\xleaders\hbox{\rule{4pt}{0pt}\rule[\dimexpr.5ex-.2pt]{4pt}{1.2pt}}\hfill\kern0pt%
}
\newcommand{\mythickdashrule}[0]{%
\\[-2\jot]
\multicolumn{4}{@{}c@{}}{\makebox[\linewidth]{\thickdashrule[black!60]}} \\[-\jot]}


==> tabs/acc_by_arc_len.tex <==
\begin{figure}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}[scale=1]
    \begin{axis}[ybar,
        xlabel= Distance,
        ylabel= Accuracy (\%),
        y label style={at={(axis description cs:0.05,0.5)}},
        x label style={at={(axis description cs:0.5,0)}},
        xtick=data,
        symbolic x coords={1,2,3,4,5,6,7,>=8}, 
        bar width=1.2ex, 
        xmajorgrids=true,
        ymajorgrids=true,
        legend cell align={left},
        legend style={at={(0.9,0.9)}},
        height=7cm
    ]
      \addplot [color=blue, fill=blue!80!white] 
      coordinates {
        (1,  96.36)
        (2,  96.23849539815926)
        (3,  94.70127061367938)
        (4,  93.52409638554217)
        (5, 92.42424242424242)
        (6, 89.63254593175853)
        (7, 89.55823293172691)
        (>=8, 87.63936015511391)
    };
      \addplot [color=red, fill=red!80!white] 
      coordinates {
        (1, 97.37151338982003)
        (2,  96.44515187690675)
        (3,  94.87456164014028)
        (4, 93.56460532931121)
        (5, 93.02949061662198)
        (6, 90.94540612516645)
        (7, 89.09090909090909)
        (>=8, 87.78813143697891)
    };
    \legend{\citeauthor{yang-tu-2022-headed} \\ \texttt{Hexatagger}\\}
    \end{axis}
\end{tikzpicture} }
\end{center}
\caption{}
\label{fig:acc_by_arc_len}
\end{figure}
